Explaining Deep Neural Networks by Leveraging Intrinsic Methods

Despite their impact on the society, deep neural networks are often regarded as black-box models due to their intricate structures and the absence of explanations for their decisions. This opacity poses a significant challenge to AI systems wider adoption and trustworthiness. This thesis addresses this issue by contributing to the field of eXplainable AI, focusing on enhancing the interpretability of deep neural networks. The core contributions lie in introducing novel techniques aimed at making these networks more interpretable by leveraging an analysis of their inner workings. Specifically, the contributions are threefold. Firstly, the thesis introduces designs for self-explanatory deep neural networks, such as the integration of external memory for interpretability purposes and the usage of prototype and constraint-based layers across several domains. Secondly, this research delves into novel investigations on neurons within trained deep neural networks, shedding light on overlooked phenomena related to their activation values. Lastly, the thesis conducts an analysis of the application of explanatory techniques in the field of visual analytics, exploring the maturity of their adoption and the potential of these systems to convey explanations to users effectively.

==> Include/Chapters/Graph.tex <==
\chapter{Self-Explainable Deep Graph Neural Networks}
% % \gls{ML}
% % \gls{AI}
% % \gls{DL}
% % \gls{DNN}
% % \gls{XAI}
% \gls{MANN}
% % \gls{NN}
% \gls{CNN}
% \gls{GNN}
% \gls{GCN}
% \gls{GAT}
% \gls{GIN}
% \gls{VA}
% % \gls{CoEx}
% % \gls{NetDissect}
% % \gls{PIGNN}
% % \gls{SDNC}
% % \gls{DNC}
%\newacronym{MLP}{MLP}{Multi-Layer Perceptron}
%\newacronym{CBM}{CBM}{Concept Bottleneck Models}
%\newacronym{GCW}{GCW}{Graph Concept Whitening}
This chapter explores self-explainable graph neural networks, a class of architectures that aims to address the opacity of \glspl{GNN} by integrating elements that improve their interpretability directly into their structure. 
%ADDED
Specifically, this chapter presents the generalization of two recently proposed self-explainable designs for image data to \glspl{GNN}, graph data, and the chemistry domain. As in the previous chapter, the idea is to preserve most of the black-box structure so as not to lower the performance. Specifically, we propose the addition of a prototype layer after the feature extractor and embedding constraints into the normalization process to make the decision process of neural networks more interpretable. The few existent self-explainable deep neural networks~\cite{Chen2019, Chen2020} assume the feature extractor is a \gls{DNN} already trained (i.e., the training is decoupled), and are tailored to specific architectures, domains, and tasks (i.e., vision and image classification). This chapter aims to contribute to this research area by proposing designs where both the feature extractor and the added elements can be jointly trained from scratch and their concepts can be applied to different domains (i.e., chemistry and graph data).

\input{Include/Chapters/PIGNN}
\input{Include/Chapters/ConceptWhitening}
\section{Analysis and Contributions}
This chapter contributed to the research on self-explainable neural networks by exploring their design in the emerging field of \glspl{GNN}, a field that has been mostly unexplored. Specifically, we investigated the application of prototype layers and concept whitening to graph data and in the chemical domain. We analyzed the differences and specific characteristics of the graph applications, along with the advantages and weaknesses associated with their utilization for enhancing the interpretability of \glspl{GNN}. 

Notably, both approaches preserve the performance of the black-box models while improving their interpretability in terms of fidelity with respect to their decision process. Unlike the image domain, prototype layers proved themselves to be more effective when jointly trained with the feature extractor. Moreover, they provide more sparse and easy-to-understand global and local explanations, highlighting the learned subgraphs in terms of prototypes, which are then used for the prediction, and the most important subgraph for a specific prediction. With Graph Concept Whitening, we take a step forward with respect to the approaches described in the previous chapter and in \Cref{sec:proto_design}). Instead of adding elements to the network, this approach modifies the normalization layers so that the interpretation of the learned latent space is easier, thereby improving the interpretability of the network. We discussed how this modification can also be performed in the fine-tuning stage without loss of accuracy and how to inspect the decision process of the network via the inspection of the latent space.

Alongside these strengths, we also analyzed some of the drawbacks of these approaches. For example, the number of prototypes in prototype layers represents a parameter difficult to choose that impacts both performance and quality of explanations, especially in unbalanced datasets. On the other hand, when using Graph Concept Whitening, the selection of concepts and the dependence on the prior design of the architecture (i.e., it performs better when replacing BatchNormalization layers) represent limitation to the applicability of the approach compared to all the previous approaches, which are, instead, are model-agnostic.
